Counterfactual Density Estimation using Kernel Stein Discrepancies

Causal effects are usually studied in terms of the means of counterfactual distributions, which may be insufficient in many scenarios. Given a class of densities known up to normalizing constants, we propose to model counterfactual distributions by minimizing kernel Stein discrepancies in a doubly robust manner. This enables the estimation of counterfactuals over large classes of distributions while exploiting the desired double robustness. We present a theoretical analysis of the proposed estimator, providing sufficient conditions for consistency and asymptotic normality, as well as an examination of its empirical performance.

==> spare.tex <==
    \begin{align} \nonumber
        &\text{A10)}  \iint \sup_{\theta \in \Theta} \| \frac{\partial}{\partial\theta} h_\theta^*(z, \tilde z) \|_{\R^{p}} dQ(z)dQ(\tilde z) < \infty, 
        \\\nonumber&\text{A11)} \iint \| \frac{\partial}{\partial\theta} h_\theta^*(z, \tilde z) \|_{\R^{p}}^2 dQ(z)dQ(\tilde z)\mid_{\theta = \theta_*} < \infty, \\
        &\text{A12)} \iint \sup_{\theta \in \Theta} \| \frac{\partial^2}{\partial\theta^2} h_\theta^*(z, \tilde z) \|_{\R^{p\times p}} dQ(z)dQ(\tilde z) < \infty,&&\text{A13)} \int \sup_{\theta \in \Theta} \| \frac{\partial^2}{\partial\theta^2} h_\theta^* (z, z)\|_{\R^{p\times p}} dQ(z)< \infty, \nonumber
        \\&\text{A14)} \;\Gamma := \frac{1}{2} \iint \frac{\partial^2}{\partial\theta^2} h_\theta^*(z, \tilde z)  dQ(z)dQ(\tilde z) \mid_{\theta = \theta_*} \succ 0. \nonumber
    \end{align} \nonumber


    Moreover, although we have stated Theorem \ref{theorem:normality} in terms of suprema in $\Theta$ for the interest of presentation. Nonetheless, the consistency of $\theta_n$ implies that it will be in a neighbourhood of $\theta_*$ with high probability for big enough $n$, and hence it would suffice to take suprema in any neighbourhood of $\theta_*$.

    (this grid could be fix or dynamic; for instance, $\theta_{g_n}$ could correspond to the parameters investigated through stochastic gradient descent)

    While this statistic resembles the one presented in \citet{martinez2023efficient}, several important differences arise between the two. First and foremost, \citet{martinez2023efficient} studied distributional treatment effects, hence the causal target itself was different. Second, their work did not extend to embeddings that depend on a parameter $\theta$. Lastly, their statistic requires sample splitting, using only half of the data on each side of the inner product. In contrast, $g_n$ uses the $n$ observations on each side, hence retaining the $\sqrt{2}$-factor in the convergence rate that is lost otherwise.

Our work extends upon a statistic introduced in these prior contributions.  \cite{fawkes2022doubly} and \cite{martinez2023efficient} studied the distribution of this statistic under the null in order to calibrate a two-sample test. In contrast, our approach suggests minimizing a similar statistic within a specific class of distributions in order to model the counterfactual. Both the motivation and theoretical challenges in our study diverge from those in the earlier works; we view our research as complementary and orthogonal to these previous contributions.

    \STATE Choose kernel $k$ and estimators $\hat{\beta}$, $\hat{\pi}$. 
    \STATE Split data in two sets  $\mathcal{D}_1 = (X_i, A_i, Y_i)_{i = 1}^{n//2}$ and $\mathcal{D}_2 = (X_i, A_i, Y_i)_{i = n//2+1}^{n}$. 
    \STATE Train $\hat\pi^{(1)}$, $\hat\beta^{(1)}$ on $\mathcal{D}_2$ and $\hat\pi^{(2)}$, $\hat\beta^{(2)}$ on $\mathcal{D}_1$. Take $\hat\pi$, $\hat\beta$ as $\hat\pi^{(r)}$, $\hat\beta^{(r)}$ on $\mathcal{D}_r$ for $r \in \{1, 2 \}$.
    \STATE Define $\hat{\beta}_\theta$ from $\hat{\beta}$ as in \eqref{eq:betathetahat}, and $\hat\phi_\theta$ as the plug-in estimate of \eqref{eq:phidef} using $\hat{\beta}_\theta$ and $\hat{\pi}$.
    \STATE Define $g_n$ as in \eqref{eq:statistic}.
    \STATE Take $\theta_n \in \arg\min_{\theta \in \Theta} g_n(\theta; Y_1, \ldots, Y_n)$.
    \STATE \textbf{return} $p_{\theta_n}$.



    We note that $Q_n \hat\phi_\theta - Q_n \phi_\theta = T_1(\theta) + T_2(\theta)$, where $T_1(\theta) = (Q_n - Q)(\hat\phi_\theta - \phi_\theta)$ and $T_2(\theta) = Q(\hat\phi_\theta - \phi_\theta)$. Following again \citet[Lemma C.7]{martinez2023efficient} and the arguments in \citet[Theorem C.9]{martinez2023efficient}, we deduce that 
\begin{align} \nonumber
    \|T_1(\theta)\|_{\mathcal{H}^d} \leq O\left(\frac{\| \hat\phi_\theta - \phi_\theta \|}{\sqrt{n}}\right), \quad \|T_2(\theta)\|_{\mathcal{H}^d} \leq \frac{1}{\epsilon} \| \pi - \hat\pi\| \|\beta_\theta - \hat\beta_\theta \|. 
\end{align}
Given that $\sup_{\theta \in \Theta}\| \hat \phi_\theta - \phi_\theta\| = o(1)$ and $\|\hat\pi - \pi\| \sup_{\theta \in \Theta}\left\{\|  \hat\beta_\theta - \beta_\theta \|\right\} = o(\frac{1}{\sqrt{n}})$, we arrive to $\sup_{\theta \in \Theta}\|Q_n \hat\phi_\theta - Q_n \phi_\theta\|_{\mathcal{H}^d} = o(\frac{1}{\sqrt{n}}) + o(\frac{1}{\sqrt{n}}) = o(\frac{1}{\sqrt{n}})$. With an analogous argument by replacing $\hat\phi_\theta$ by $\frac{\partial}{\partial\theta}\hat\phi_\theta$ and $\phi_\theta$ by $\frac{\partial}{\partial\theta}\phi_\theta$, we derive that 
\begin{align} \nonumber
    \sup_{\theta \in \Theta}\|\frac{\partial}{\partial\theta} \left\{Q_n \hat\phi_\theta - Q_n \phi_\theta \right\}\|_{\mathcal{H}^d} = \sup_{\theta \in \Theta}\|Q_n \frac{\partial}{\partial\theta} \hat\phi_\theta - Q_n \frac{\partial}{\partial\theta} \phi_\theta \|_{\mathcal{H}^d} = o(\frac{1}{\sqrt{n}}),
\end{align}
based on assumptions $\sup_{\theta \in \Theta}\| \frac{\partial}{\partial\theta}\hat \phi_\theta - \frac{\partial}{\partial\theta}\phi_\theta\| = o(1)$ and $\|\frac{\partial}{\partial\theta}\hat\pi - \pi\| \sup_{\theta \in \Theta}\left\{\| \frac{\partial}{\partial\theta} \hat\beta_\theta - \frac{\partial}{\partial\theta}\beta_\theta \|\right\} = o(\frac{1}{\sqrt{n}})$.

The uniform consistency of the estimator for $\phi_\theta$ is implicitly exploited in the proof of Theorem \ref{theorem:consistency}, and analogous arguments would carry for the $\partial_\theta\phi_\theta$ case under the assumptions of Theorem \ref{theorem:normality}.
